MTEB-French: Resources for French Sentence Embedding Evaluation and Analysis

Recently, numerous embedding models have been made available and widely used for various NLP tasks. The Massive Text Embedding Benchmark (MTEB) has primarily simplified the process of choosing a model that performs well for several tasks in English, but extensions to other languages remain challenging. This is why we expand MTEB to propose the first massive benchmark of sentence embeddings for French. We gather 15 existing datasets in an easy-to-use interface and create three new French datasets for a global evaluation of 8 task categories. We compare 51 carefully selected embedding models on a large scale, conduct comprehensive statistical tests, and analyze the correlation between model performance and many of their characteristics. We find out that even if no model is the best on all tasks, large multilingual models pre-trained on sentence similarity perform exceptionally well. Our work comes with open-source code, new datasets and a public leaderboard.

==> paper_sections/old_datasets.tex <==
We identified 8 datasets relevant to French in the existing MTEB. We complemented these with 14 external relevant datasets and created three new ones. Therefore, as of today, our French MTEB runs on 25 datasets (see Figure \ref{fig:PCA_similarity}) spread over all aforementioned tasks. This section describes the 3 new datasets we introduce and analyses the similarities between datasets.

\subsubsection{New datasets}
\label{sec:new_datasets}

    \textbf{Syntec (Retrieval)}
    % add ref to appendix quality checks
    The Syntec French collective bargaining agreement\footnote{\url{https://www.syntec.fr/convention-collective/}} comprises around 90 articles. 
    Despite its topic, the language used does not feature the specificity of the legal vocabulary, making the data suitable for benchmarking general-purpose models. 
    The articles have been scraped for use as documents. 
    Four annotators, not experts in employment law, were divided into two groups. 
    Each group was given half of the articles and asked to choose an article and write a question about it. 
    Each annotator wrote 25 questions. 
    Thus, a hundred questions have been manually created and paired with the articles containing the answer\footnote{The link to the publicly accessible dataset on Hugging Face will be added once the anonymization process is complete.}.
    %\footnote{\url{https://huggingface.co/datasets/lyon-nlp/mteb-fr-retrieval-syntec-s2p}}.
    Examples of the dataset are available in the appendix Figure \ref{fig:extract-syntec}.
    This dataset could also be used for text classification, clustering or topic modeling. 
    

    \textbf{HAL (Clustering)}
    % add ref to appendix quality checks
    \emph{Hyper Articles en Ligne} (HAL) is a French open archive of scholarly documents from all academic fields. 
    Scrapping this resource, we fetched 85,000 publications in French\footnote{The link to the publicly accessible dataset on Hugging Face will be added once the anonymization process is complete.}. 
    We extracted titles and domains labels.
    The latest are provided by authors when submitting their papers to HAL.
    And since annotations (human labeled) are provided, the dataset can be used for many tasks such as topic modeling or text classification.
    To ensure the dataset quality is suitable for a benchmark, further cleaning of data has been performed : 
    1) Duplicates are eliminated, retaining unique publications for each field. 
    2) Irrelevant titles (due to API indexing mistakes) or title in languages other than French have been manually removed.
    3) Samples belonging to \emph{domain} classes with less than 500 samples were removed, which leads us to keep only 10 classes. 
    4) Subsampling was performed on 2 classes containing more than 10k samples each, in order to lower the number of samples and mitigate the unbalance of the dataset. 
    More details about this process are provided in the appendix \ref{app:hal} along with some extracts in Figure \ref{fig:extract-hal}.
    We make the dataset available in both their raw and clean versions. 
    We use this dataset in a clustering setup, where we cluster publications by their title and use the domain as ground truth.


    \textbf{SummEvalFr (Summarization)}
    % add ref to appendix quality checks
    The original SummEval dataset \cite{fabbri2021summeval} consists of 100 news articles from the CNN/DailyMail dataset. 
    Each article has 11 human-written summaries and 16 machine-generated summaries annotated by eight persons with a score for coherence, consistency, fluency, and relevance. 
    We translated it from English to French using DeepL API\footnote{\url{https://www.deepl.com}}.
    We have not added any annotations. 
    This dataset can now be used for translation by combining it with its English homologue. We provide a detailed quality checking process in section \ref{sec:quality}.

\textbf{Reranking datasets}
The reranking task, as evaluated in MTEB, requires datasets composed of a set of queries, each associated with relevant and irrelevant documents. Despite our efforts, we found no French dataset that natively exhibits such a structure. Thus, to evaluate this task, we built reranking datasets based on the \textit{Syntec} and \textit{Alloprof} \cite{lef23} retrieval datasets. These already feature queries and labeled relevant documents. Irrelevant ones were added using the following process. In order to avoid bias, we use the BM25 algorithm \cite{Robertson1976RelevanceWO} (which is a deterministic method) to rank documents for each query. The top 10 documents that are not labeled as relevant constitute the negative samples.

We recognize that this process leads to a high correlation between the retrieval and reranking tasks. We still think it is essential to make the latter available, with an open door to future improvement.

\subsubsection{Quality checks of datasets}\label{sec:quality}
In this work, we gathered 8 existing datasets from MTEB \cite{Muennighoff2022MTEBMT}, which we assume are of good quality. 
We additionally include datasets that have been proposed in the literature such as BSARD \cite{louis2022statutory} and Alloprof \cite{lef23}, which are proven to be of good quality.
Finally, to asses of the quality of each new dataset we propose, we propose the following procedures and metrics.

\textbf{Syntec} Concerning the Syntec dataset, every article has been reviewed while manually creating a question about it. Moreover, it has been checked that each question can be answered by only one specific document.

\textbf{HAL} To ensure the quality of this dataset, in addition to the cleaning procedures presented in \ref{sec:new_datasets}, we run 3 baseline models for classification on HAL: \emph{TF-IDF + SVM}, a fine-tuned \emph{cammebert} \cite{Martin2019CamemBERTAT} and \emph{GPT-4} leveraging In-Context Learning (ICL). Additionally, we run one baseline model for topic modeling: Latent Dirichlet Allocation (LDA) \cite{blei2003latent} and report scores in the appendix \ref{app:hal}.

\textbf{SummEvalFr} For the summarization dataset, since MTEB evaluation is based on embedding similarity between machine-generated and human-generated summaries, we propose to compute the ROUGE \cite{lin2004rouge} and BLEU \cite{papineni2002bleu} metrics between them for both French and English. 
In Table \ref{tab:rouge_bleu}, we report the average of the scores as well as their correlations between the two languages. The correlation is high (above 0.7) showing that the word and n-gram overlap between human and machine summaries is highly preserved in the French version.\\
One may argue that computing the metric on fully translated texts (human and machine summaries are both translated from English), may introduce biases and do not asses of the quality of the translations. 
For this purpose, we make sure the translated human summaries are correctly translated. 
We use a LLM as-a-judge \cite{zheng2023judging} (see \ref{app:summeval} for the prompt), where given the original human summary in English and its translation in French, the model rates the quality of the translation from $0$ to $10$, with $0$ being of very bad quality and $10$ being excellent. 
We check manually random translations with ratings between 9 and 10 to make sure the rating is relevant. 
Then we then check manually all translations with a score less than $9$ and correct them (see the distribution of ratings in \ref{app:summeval}). 

\begin{table}[h]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccc}
        \hline
        \textbf{Dataset} & \textbf{BLEU} & \textbf{ROUGE-1} & \textbf{ROUGE-2} & \textbf{ROUGE-L}  \\
        \hline
        SummEval & 0.205 & 0.292 & 0.099 & 0.193 \\
        %\hline
        SummEvalFr & 0.276 & 0.302  & 0.117 & 0.194 \\
        %\hline
        Correlation En-Fr & 0.70 & 0.85 & 0.80 & 0.84 \\
        \hline
    \end{tabular}
    }
    \caption{Average ROUGE and BLUE scores computed between machine summaries and human summaries for the original English SummEval and its translation to French. The correlations of the individual scores between English and French are also reported.}
    \label{tab:rouge_bleu}
\end{table}

In addition to all performed checks, we run multiple models on these datasets and provide results to show that these datasets are neither trivial nor impossible to solve (see tables \ref{tab:res_classif_pairclassif}, \ref{tab:res_bitext_reranking_retrieval} and \ref{tab:res_clustering_summarization}).

\subsubsection{Similarity analysis}
\label{sec:dataset_sim}
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/PCA_similarity.png}
    \caption{2D projection of datasets. 90 random samples per dataset are embedded using \emph{multlingual-e5-large} model \cite{wang2022text}. The embeddings are reduced to 2 dimensions using PCA. The centroid of each dataset is represented, along with the ellipse showing the standard deviation along each axis.}
    \label{fig:PCA_similarity}
\end{figure*}

We investigate the proximity between the datasets' topics to give insights about the benchmark contents. 
The methodology introduced by \citet{Muennighoff2022MTEBMT}, i.e. computing a sampled average embedding of the datasets, is used to build a dataset-similarity matrix (displayed in appendix Figure \ref{fig:cosine_similarity}).
The distances between averaged embedding vectors of each dataset (which range from $0.89$ to $1$ in Figure \ref{fig:cosine_similarity}) remains hard to interpret into a dataset semantic proximity. Thus, we complement this by observing the dataset's clouds of embedding in a 2D plane using PCA in Figure \ref{fig:PCA_similarity}.

Figures \ref{fig:PCA_similarity} and \ref{fig:cosine_similarity} seem to correlate, showing high similarity between two datasets when the same underlying data is used in different tasks. 
Dataset topics are pretty close, with some exceptions, such as the Syntec dataset.
As more datasets are added to the benchmark, this analysis will help select new data that do not produce redundant results. It may also help to understand the link between the results and the datasets' topics.

==> paper_sections/old_introduction.tex <==
Embeddings are dense vector representations that capture the semantics of an input. 
The first emblematic example is Word2Vec, introduced by \citet{Mikolov2013EfficientEO}. It consists of neural architectures trained to learn high-quality word representations from contextual relationships in vast amounts of text. 
Other models were proposed since then, leveraging the transformer architecture \citep{Vaswani2017AttentionIA} to produce both generic and contextualized word embeddings using self-attention.
The most influential one is BERT \citep{Devlin2019BERTPO}, a transformer-based encoder pre-trained on the Masked-Language Modeling and Next Sentence Prediction tasks to learn the semantics of a language. 
Many models now exist with various architectures, monolingual or multilingual, pre-trained or fine-tuned \citep{naseem2021comprehensive, ding2023sentence}. 
Embeddings are essential for many NLP applications, such as semantic search, topic modeling, classification, etc.
Choosing the most suitable model for a specific application is not always obvious. 
Hence, initiatives such as MTEB \citep{Muennighoff2022MTEBMT} enable these models to be compared across various datasets and tasks.
However, most of the provided resources for the evaluations are in English. 

We extend MTEB to produce the first massive benchmark on French embeddings.
Our contributions are the following. 
We bring together 25 datasets (3 of which are new) in an easy-to-use toolbox. We compare 46 models with diverse characteristics on a large scale. We propose an in-depth performance analysis based on model characteristics, statistical tests, and a meta-analysis of all language-specific MTEB leaderboards. 

Although no model is the best on all tasks, a set of methods performs exceptionally well for most benchmark datasets (see Figure \ref{fig:crit_diff_diagram}).
We also find a strong correlation between a model's performance, its size, its training technique, and the use of multilingual data. 
%Our open-source code and results are publicly available on the MTEB repository and leaderboard \url{https://github.com/embeddings-benchmark/mteb}.
The code and all the resources used for this work are publicly available as open-source. 

==> paper_sections/old_related_work.tex <==
This section first describes the various family of models used in this benchmark. 
Previous works comparing embedding models are also discussed. 

    \subsection{Sentence embeddings}
    Sentence embeddings are required for a large set of language tasks, such as Semantic Textual Similarity (STS) and knowledge retrieval. 
    Before the standardization of the transformer architecture \citep{Vaswani2017AttentionIA}, the common architecture used to obtain sentence embeddings was Recurrent Neural Networks (RNN) \citep{kiros2015skip}. Many models have been proposed to build sentence representations leveraging this architecture, for example, \emph{LASER} \citep{Artetxe2018MassivelyMS} which trains a BiLSTM encoder and a LSTM decoder to produce multilingual sentence embeddings.   
    
    Now that most language models leverage the transformer architecture, a large majority of embedding methods internally start by generating embeddings for tokens. An additional step is therefore required to compute sentence embeddings. A well-known strategy is pooling, which can be done either using the embedding of the CLS token \citep{Devlin2019BERTPO}, or by mean-pooling which averages the tokens output vector representations. Alternatively, max-pooling is sometimes used and consists in taking the component-wise maximum across all token embeddings. Finally, for sequential and causal models, the common strategy is to use the last token representation \citep{muennighoff2022sgpt}.
    %A well-known strategy is pooling, which can be achieved leveraging multiple approaches. 
    %One consists of using the embedding of the CLS token \cite{Devlin2019BERTPO} produced by BERT-like models, which constitutes the sentence-level representation.
    %Another one is mean-pooling where the sentence embedding is calculated by averaging its words output vector representations. 
    %The latest one is max-pooling, where we take the output vector representation of the token with the largest values. 
    
    In addition to pooling, these embeddings can be learned by training a siamese network which outputs vector representations that can be compared using similarity measure \citep{Reimers2019SentenceBERTSE}.
    For encoder-decoder based language models that do not come with a CLS token such as \emph{T5} \citep{Raffel2019ExploringTL}, authors like \citet{ni2021sentencet5} propose to train a dual encoder paired with a contrastive learning framework \citep{Gao2021SimCSESC, neelakantan2022text}. 
    %However, T5-based models are monolingual and are only trained on English texts. 
    Other works build multilingual models leveraging contrastive frameworks on sentence similarity such as \emph{E5} \citep{wang2022text}.
    
    More recently, Large Language Models (LLM) have been used to build sentence embeddings, also through fine-tuning on sentence similarity \cite{wang2023improving, Zhang2023LanguageMA}. Some of these models are not openly accessible, namely OpenAI's \emph{text-embedding-ada-002}\footnote{\url{https://platform.openai.com/docs/guides/embeddings/embedding-models}}, or Cohere\footnote{\url{https://txt.cohere.com/introducing-embed-v3/}} and Voyage models\footnote{\url{https://docs.voyageai.com/embeddings/}}.
    %With the revolution of Large Language Models (LLM), researchers have built embeddings that leverage the semantics learned by these large models \citep{muennighoff2022sgpt}.
    %We distinguish two categories of LLMs, closed-source models and open-source ones.
    %The first ones are not openly accessible and are built upon private models such as \emph{GPT-3} \cite{brown2020language, ouyang2022training}.
    %They gained in popularity due to their ease of use (API calls and no model deployment management). 
    %The most used models to this day are \emph{text-embedding-ada-002} from OpenAI\footnote{\url{https://platform.openai.com/docs/guides/embeddings/embedding-models}}, Cohere embeddings\footnote{\url{https://txt.cohere.com/introducing-embed-v3/}} and Voyage ones\footnote{\url{https://docs.voyageai.com/embeddings/}}.
    %For open-source models, a large panoply of them was made available by some organizations and researchers.
    %The first models to compete with \emph{GPT-3.5} were the \emph{Llama} family of models \cite{touvron2023llama, touvron2023llama2}.
    %Initiatives fine-tune open-source LLM on sentence similarity \cite{wang2023improving, Zhang2023LanguageMA} and show that they can be competitive with other models.

    % French BERT variants, keep it at the end
    Regarding the French-specific literature, models based on the BERT architecture were proposed by the community, such as \emph{camemBERT} \cite{Martin2019CamemBERTAT}, \emph{flauBERT} \cite{le2020flaubert}, and very recently larger models such as \emph{Vigogne}\footnote{\url{https://github.com/bofenghuang/vigogne}} and \emph{CroissantLLM} \cite{faysse2024croissantllm}.

    \subsection{Benchmarks}
    % Marion
    Embedding models are generally compared on specific tasks.
    For example, BEIR \cite{Thakur2021BEIR} focuses on Information Retrieval, while SemEval \cite{Agirre2016Semeval} is used for STS. The Reranking task is also considered in some benchmarks \cite{Wang2021Tsdae}. 
    Others works evaluate embedding models on multiple tasks such as GLUE \cite{Wang2018GLUEAM}, BIG-bench \cite{Srivastava2022BeyondTI}, SentEval \cite{Conneau2018SentEval} or the meta-embeddings comparison \cite{Garcia2021Bench}.
    
    The most comprehensive benchmark to date is MTEB \cite{Muennighoff2022MTEBMT}.
    It compares 33 models across 8 embedding tasks on 58 datasets, allowing to take informed decision when selecting an embedding model. 
    It results in no model is best on all tasks. 
    Therefore, the different embedding models seem to exhibit task-dependent strengths and weaknesses. 
    Performance is also strongly correlated with the model size, so users can define their trade-off between efficiency (speed, memory) and embedding quality. 
    They can also have other criteria such as multilingualism. 
    The MTEB benchmark mainly focuses on sentence embeddings. 
    It attempts to select tasks that resemble downstream applications (such as retrieval, classification, clustering, etc.) in order to help the user project into such use-cases. 
    However, it should be kept in mind that the datasets may not perfectly reflect the peculiarity of the downstream tasks.
    
    MTEB still has an important limit: it does not easily allow to select a model for other languages than English or for multilingual applications.
    Some initiatives already evaluate embedding models for specific languages, such as Arabic \cite{Elnagar2023Arabic} and German \cite{Wehrli2024German}.
    Our work comes with the same ambition for French.
    It relies on the MTEB structure that provides a solid basis for analysis, and extend it to a new language.  
    
    % Discuss original MTEB
    %We propose this work to extend the MTEB benchmark \cite{Muennighoff2022MTEBMT}. 
    %Their work compares 33 models on 8 embedding tasks with 58 datasets, allowing to take informed decision when selecting an embedding model. 
    %It results in no model with state-of-the-art performance on all tasks. 
    %Therefore, the different embedding models seem to exhibit task-dependent strengths and weaknesses. 
    %Performance is also strongly correlated with the model size, so users must define their trade-off between efficiency (speed, memory) and embedding quality. 
    %They can also have other criteria such as multilingualism. 
    %A large gap remains between self-supervised and supervised methods.
    %Their work provides a solid basis for further analysis.
    %The MTEB benchmark mainly focuses on text embeddings (and not words). 
    %It attempts to select tasks that resemble downstream applications (such as retrieval, classification, clustering, etc.) in order to help the user plan for these uses. 
    %However, it should be kept in mind that the datasets may not perfectly reflect the peculiarity of the downstream tasks.

    %Benchmarks on specific tasks
    %Other benchmarks already evaluated embedding models such as GLUE \cite{Wang2018GLUEAM}, BIG-bench \cite{Srivastava2022BeyondTI}, SentEval \cite{Conneau2018SentEval} or the meta-embeddings comparison \cite{Garcia2021Bench}.
    %Specific tasks can also be assessed. 
    %For example, BEIR \cite{Thakur2021BEIR} focuses on Information Retrieval, while SemEval \cite{Agirre2016Semeval} is used for Semantic Textual Similarity (STS) and the Re-Ranking task is also considered \cite{Wang2021Tsdae}. 
    %Some of these datasets are included in the MTEB benchmark.
    
    %Benchmarks on specific languages
    %More initiatives evaluate embedding models for specific languages, such as Arabic \cite{Elnagar2023Arabic} and German \cite{Wehrli2024German}.
    %Our work comes with the same ambition for French. 
    

==> paper_sections/old_tasks.tex <==
\subsection{Tasks}
As stated in the original paper \citep{Muennighoff2022MTEBMT}, MTEB evaluates the ability of models to produce relevant embedding vectors in the context of 8 different tasks. This section goes through each of them.

\paragraph{Bitext Mining}
This tasks requires two sets of sentences, each in a different language. Given a sentences from the first set, this tasks aims at finding the best match in the second set. The match is generally a translation. This task evaluates the ability of a multilingual model to produce embedding vectors that are close in distance when the meaning of the sentence is the same, despite the language being different. The main metric used for this task is f1-score.

\paragraph{Classification}
The classification task requires a set of texts along with their annotated class. The texts are split into train and test sets that are embed using the model to evaluate. The embed train set is then used to train a logistic regression classifier for a maximum of 100 iterations. The classifier is then scored on the test set using accuracy with average precision metric, and F1-score. Intuitively, this task evaluate the ability of the embedding model to produce embedding vectors that carry close representations of texts within a class. These representations shall allow to train performant logitic regression classifier.

\paragraph{Clustering}
Similarly to the classification task, the clustering task aims at evaluating if the embedding model is able to help with subdividing a set of texts into meaningful clusters. Consequently, a set of labeled text is also required for this task. For the purpose of the evaluation, a mini-batch k-means model with batch 32 and k equals to the number of different labels is trained one the embedded texts. The model is score using v-measure, so that the metric is not impacted by the mismatch between class and cluster label.

\paragraph{Pair classification}
This tasks requires a set of text pairs annotated with a label. The label typically is binary and indicates whether the pair is a paraphrase, or a duplicate. For the evaluation of the model, both texts of the pair are embed using a model. The distance between both vector is then computed with cosine similarity, euclidean distance, dot product and Manhattan distance. Using the best binary threshold, accuracy, average precision, f1-score, precision and recall are computed, with average precision score based on cosine similarity being the main metric.

\paragraph{Reranking}
The reranking task requires a text (referred to as a query) associated with a small set of text (referred to as the documents). The goal of this task is to rank the set of documents in terms of relevance regarding to the query. To this end, the query and each documents are embed using the model to evaluate. The embedding of the query is compared with each document using cosine similarity. In other words, the model is evaluated based on its ability to produce vectors for which their distance with the query is correlated with their relevance.The metrics used are mean MRR@k and MAP, with MAP being the main metric.

\paragraph{Retrieval}
This is a praragraph

\paragraph{Semantic textual similarity}

\paragraph{Summarization}

==> paper_sections/tasks.tex <==
Similarly to MTEB \citep{Muennighoff2022MTEBMT}, we evaluate the ability of models to produce relevant embedding vectors for 8 different tasks :
\\
\textbf{Bitext Mining} evaluates a model's ability to produce vector representations that preserve the semantics of a pair of sentences from different languages.
\\
\textbf{Classification} ensures that an embedding model produces vectors that help classifiers correctly associate samples to their relevant classes. 
\\
\textbf{Clustering} ensures clusters of semantically close sentences can be built based on their embeddings.
\\
\textbf{Pair Classification} assesses whether a model generates close vector representations for texts that carry the same information, and distant ones for texts that do not.
\\
\textbf{Retrieval} implies that a model creates documents and queries embeddings for which the distance is correlated with matching relevance.
\\
\textbf{Reranking} assesses whether a model produces embeddings that enable ordering documents according to their relevance regarding a given query.
\\
\textbf{Semantic Textual Similarity (STS)} evaluates the ability to generate representations for which the distance between texts determine their relatedness.
\\
\textbf{Summarization} evaluates the ability of a model to produce embedding vectors for both a text and its summary that are close if the summary is relevant.


More information about the tasks can be found in the MTEB paper \citep{Muennighoff2022MTEBMT}. Overall, most tasks have in common that they evaluate the relevance of embedding similarity in different contexts.


==> tables/multilingual_avg_performance.tex <==
\begin{table}[htbp]
\centering 
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr}
\hline
\multicolumn{1}{c}{\textbf{Model}} & 
 \multicolumn{4}{c}{\textbf{Normalized rank in \% (rel. rank)}} \\
 &
\textbf{FR} & \textbf{EN} & \textbf{ZH} & \textbf{PL}\\
\hline
\emph{text-embedding-3-large} & 1 (1) & 17 (4) & 66  (6)& - \\
\emph{text-embedding-3-small} & 2 (2) & 42 (4) & 66  (6)& - \\
\emph{text-embedding-ada-002} & 3 (3) & 59 (4) & 66  (6)& - \\
\emph{bge-m3} & 2 (3) & 22 (4) & 66  (6)& - \\
\emph{mistral-embed} & 52 (14) & 2 (1) & 46 (1) & -\\
\emph{e5-mistral-7b-instruct} & 52 (14) & 8 (1) & 46 (1) & -\\
\emph{sentence-t5-xxl} & 4 (2) & 72 (6) & - & - \\
\emph{multilingual-e5-large} & 9 (3) & 19 (3) & 52 (2) & 22 (1)\\
% \emph{Cohere-multilingual-v3} & 11 (4) & 5 (2) & - & -\\
\emph{multilingual-e5-base} & 13 (5) & 73 (7) & 60 (3) & 44 (2)\\
% \emph{sentence-t5-xl} & 17 (6) & 38 (10) & - & -\\
\emph{multilingual-e5-small} & 20 (7) & 38 (9) & 62 (4) & 50 (3)\\
\emph{paraph-multi-mpnet-base-v2} & 22 (8) & - & 78 (8) & 72 (4)\\
% \emph{Cohere-multilingual-light-v3} & 24 (9) & 25 (5) & - & -\\
% \emph{sentence-t5-large} & 33 (10) & 42 (11) & - & -\\
% \emph{LaBSE} & 39 (11) & 58 (14) & - & 83 (5)\\
% \emph{sentence-t5-base} & 43 (12) & 50 (13) & - & -\\
% \emph{laser2} & 50 (13) & 62 (15) & - & - \\
\emph{udever-bloom-1b1} & 59 (15) & 34 (8) & 64 (5) & -\\
\emph{udever-bloom-560m} & 91 (16) & 48 (12) & 68 (7) & -\\
\hline
\end{tabular}
}
\caption[Caption for LOF]{Ranking of models according to their average performance over all tasks in French (FR), English (EN), Chinese (ZH) and Polish (PL). The first value corresponds to a normalized rank computed by dividing the rank of the model compared to its competitors on a language, by the total number of evaluated models for this language. This total number is 46, 141, 60 and 18 respectively for French, English, Chinese and Polish. The normalized rank can be interpreted as a quantile, \emph{e.g.} \emph{text-embedding-ada-002} is in the top 2 percent quantile for French. The value in parenthesis is the relative rank between the models in the table only.}
\label{tab:multi_avg_perf}
\end{table}



==> tables/table_results.tex <==
\begin{table*}[htbp]
%\th.col-1left
\begin{tabular}{lccccccccccccccccccccccc}
\hline
 & \multicolumn{6}{r}{Classification} & \multicolumn{7}{r}{Clustering} & PairClassification & \multicolumn{2}{r}{Reranking} & \multicolumn{3}{r}{Retrieval} & \multicolumn{3}{r}{STS} & Summarization \\
 Model & \rotate{AmazonReviewsClassification} & \rotate{MasakhaNEWSClassification} & \rotate{MassiveIntentClassification} & \rotate{MassiveScenarioClassification} & \rotate{MTOPDomainClassification} & \rotate{MTOPIntentClassification} & \rotate{AlloProfClusteringP2P} & \rotate{AlloProfClusteringS2S} & \rotate{HALClusteringS2S} & \rotate{MasakhaNEWSClusteringP2P} & \rotate{MasakhaNEWSClusteringS2S} & \rotate{MLSUMClusteringP2P} & \rotate{MLSUMClusteringS2S} & \rotate{OpusparcusPC} & \rotate{AlloprofReranking} & \rotate{SyntecReranking} & \rotate{AlloprofRetrieval} & \rotate{BSARDRetrieval} & \rotate{SyntecRetrieval} & \rotate{SICKFr} & \rotate{STS22} & \rotate{STSBenchmarkMultilingualSTS} & \rotate{SummEvalFr} \\
 \hline
% &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
bert-base-10lang-cased &  0.29 &  - &  0.37 &  0.44 &  0.636486 &  0.378703 &  0.532162 &  0.429190 &  0.199385 &  0.226976 &  0.193929 &  0.409573 &  0.318688 &  - &  0.362098 &  0.532500 &  0.016040 &  0.000680 &  0.138410 &  0.587641 &  0.403145 &  0.522499 &  - \\
bert-base-15lang-cased &  0.293500 &  - &  0.372831 &  0.444687 &  0.637018 &  0.378547 &  0.531617 &  0.434261 &  0.202595 &  0.227566 &  0.196732 &  0.412197 &  0.318831 &  - &  0.362073 &  0.532500 &  0.016100 &  0.000720 &  0.138410 &  0.587726 &  0.403993 &  0.522482 &  - \\
bert-base-25lang-cased &  0.293880 &  - &  0.372966 &  0.444687 &  0.636267 &  0.378578 &  0.534871 &  0.431008 &  0.197779 &  0.227605 &  0.195051 &  0.407282 &  0.319383 &  - &  0.362523 &  0.532500 &  0.016040 &  0.000710 &  0.138410 &  0.587596 &  0.387722 &  0.522499 &  - \\
distilbert-base-25lang-cased &  0.285360 &  - &  0.349529 &  0.441829 &  0.619136 &  0.353461 &  0.571429 &  0.434824 &  0.186158 &  0.252924 &  0.217762 &  0.409079 &  0.312664 &  - &  0.320008 &  0.524167 &  0.014140 &  0.000000 &  0.156150 &  0.616404 &  0.413540 &  0.570176 &  - \\
distilbert-base-en-fr-cased &  0.285120 &  - &  0.347882 &  0.440148 &  0.619198 &  0.353586 &  0.566594 &  0.421532 &  0.195433 &  0.248627 &  0.237425 &  0.407183 &  0.314329 &  - &  0.320908 &  0.524167 &  0.013640 &  0.000000 &  0.156150 &  0.616563 &  0.421808 &  0.570655 &  - \\
distilbert-base-en-fr-es-pt-it-cased &  0.285600 &  - &  0.349126 &  0.441661 &  0.619261 &  0.354150 &  0.565657 &  0.434864 &  0.195516 &  0.267024 &  0.215555 &  0.409163 &  0.310995 &  - &  0.320653 &  0.524167 &  0.014060 &  0.000000 &  0.156150 &  0.616404 &  0.415916 &  0.570473 &  - \\
distilbert-base-fr-cased &  0.285960 &  - &  0.349328 &  0.437861 &  0.617069 &  0.352740 &  0.572872 &  0.430016 &  0.196040 &  0.263846 &  0.224540 &  0.407494 &  0.314107 &  - &  0.323069 &  0.519167 &  0.013860 &  0.000000 &  0.152460 &  0.616858 &  0.428248 &  0.570303 &  - \\
bert-base-multilingual-cased &  0.293940 &  - &  0.372999 &  0.444654 &  0.636110 &  0.378359 &  0.514965 &  0.430565 &  0.208076 &  0.229340 &  0.203046 &  0.409037 &  0.317968 &  - &  0.362347 &  0.532500 &  0.016260 &  0.000710 &  0.138410 &  0.587481 &  0.390453 &  0.522472 &  - \\
bert-base-multilingual-uncased &  0.290240 &  - &  0.380061 &  0.436315 &  0.644911 &  0.394018 &  0.606615 &  0.350540 &  0.208982 &  0.337947 &  0.218354 &  0.434952 &  0.309877 &  - &  0.388493 &  0.664000 &  0.055060 &  0.000000 &  0.274840 &  0.582645 &  0.564746 &  0.549735 &  - \\
camembert-base &  0.298140 &  - &  0.309516 &  0.394855 &  0.583934 &  0.286126 &  0.542389 &  0.291880 &  0.135095 &  0.247714 &  0.125673 &  0.406021 &  0.266340 &  - &  0.242871 &  0.412667 &  0.002350 &  0.000000 &  0.048530 &  0.536831 &  0.610743 &  0.548642 &  - \\
camembert-large &  0.311680 &  - &  0.362038 &  0.463349 &  0.683934 &  0.424961 &  0.592712 &  0.342450 &  0.183866 &  0.314684 &  0.261790 &  0.440822 &  0.351463 &  - &  0.330690 &  0.510500 &  0.019680 &  0.000680 &  0.134150 &  0.588021 &  0.572576 &  0.618358 &  - \\
sentence-camembert-base &  0.360260 &  - &  0.515938 &  0.612777 &  0.771030 &  0.434388 &  0.590920 &  0.389168 &  0.202155 &  0.273037 &  0.160883 &  0.359764 &  0.270534 &  - &  0.486809 &  0.797500 &  0.219380 &  0.000000 &  0.654390 &  0.741782 &  0.775395 &  0.816390 &  - \\
sentence-camembert-large &  0.379700 &  - &  0.626530 &  0.692905 &  0.857376 &  0.586157 &  0.626880 &  0.420608 &  0.239037 &  0.474373 &  0.267904 &  0.420360 &  0.322941 &  - &  0.576181 &  0.881500 &  0.316230 &  0.000000 &  0.794420 &  0.776968 &  0.817294 &  \textbf{0.857853} &  - \\
distilbert-base-uncased &  0.254100 &  - &  0.207666 &  0.280834 &  0.440370 &  0.205387 &  0.365485 &  0.258113 &  0.122371 &  0.154455 &  0.118548 &  0.319491 &  0.243012 &  - &  0.239551 &  0.463667 &  0.004500 &  0.001480 &  0.068020 &  0.554683 &  0.155487 &  0.460244 &  - \\
Cohere-embed-multilingual-light-v3.0 &  0.386000 &  - &  0.563114 &  0.594956 &  0.807924 &  0.500063 &  0.619600 &  0.313567 &  0.173107 &  \textbf{0.565315} &  0.207639 &  0.427985 &  0.327245 &  - &  0.515985 &  0.880333 &  0.353940 &  0.001650 &  0.731170 &  0.755048 &  \textbf{0.827971} &  0.764802 &  - \\
Cohere-embed-multilingual-v3.0 &  0.418920 &  - &  0.629388 &  0.672932 &  0.862293 &  0.610742 &  0.635256 &  0.361759 &  0.199036 &  0.487157 &  0.228162 &  \textbf{0.450836} &  0.347527 &  - &  0.510128 &  0.857167 &  0.383610 &  0.006240 &  0.782460 &  \textbf{0.792325} &  0.827634 &  0.818439 &  - \\
flaubert\_base\_cased &  0.249040 &  - &  0.069805 &  0.114055 &  0.255496 &  0.094926 &  0.528593 &  0.144598 &  0.038546 &  0.271842 &  0.039420 &  0.390560 &  0.171306 &  - &  0.348129 &  0.558833 &  0.016280 &  0.002340 &  0.171200 &  0.538617 &  0.653667 &  0.371396 &  - \\
flaubert\_base\_uncased &  0.235180 &  - &  0.062374 &  0.109818 &  0.277419 &  0.086095 &  0.432022 &  0.129386 &  0.017956 &  0.142348 &  0.035478 &  0.332237 &  0.148976 &  - &  0.345516 &  0.571833 &  0.017190 &  0.000760 &  0.171970 &  0.419024 &  0.551505 &  0.334083 &  - \\
flaubert\_large\_cased &  0.224460 &  - &  0.164122 &  0.227169 &  0.242656 &  0.097902 &  0.408507 &  0.217556 &  0.052625 &  0.157538 &  0.054009 &  0.380904 &  0.187127 &  - &  0.262863 &  0.428000 &  0.005800 &  0.002190 &  0.010000 &  0.346043 &  0.485216 &  0.156594 &  - \\
multilingual-e5-base &  0.409440 &  - &  0.608339 &  0.664862 &  0.847855 &  0.555089 &  0.620890 &  0.329842 &  0.224815 &  0.414697 &  0.287899 &  0.434774 &  0.385286 &  - &  0.581006 &  0.854333 &  0.362130 &  0.000000 &  0.778930 &  0.762274 &  0.781298 &  0.806199 &  - \\
multilingual-e5-large &  0.419060 &  - &  0.635474 &  0.681473 &  0.864078 &  0.594300 &  0.629944 &  0.322649 &  0.224385 &  0.376550 &  0.289701 &  0.440358 &  0.376479 &  - &  0.573695 &  0.869000 &  0.381550 &  0.014060 &  0.795040 &  0.787795 &  0.795957 &  0.825331 &  - \\
multilingual-e5-small &  0.396780 &  - &  0.559684 &  0.614190 &  0.811964 &  0.460069 &  0.608856 &  0.325216 &  0.189515 &  0.437704 &  0.336829 &  0.431990 &  0.376091 &  - &  0.561688 &  0.867000 &  0.270110 &  0.001150 &  0.741210 &  0.756192 &  0.796173 &  0.793209 &  - \\
udever-bloom-1b1 &  0.351220 &  - &  0.432112 &  0.497814 &  0.692421 &  0.512496 &  0.622240 &  0.270566 &  0.138631 &  0.447728 &  0.213969 &  0.441146 &  0.304660 &  - &  0.391305 &  0.625833 &  0.123680 &  0.000000 &  0.362190 &  0.599425 &  0.771042 &  0.499729 &  - \\
udever-bloom-560m &  0.268500 &  - &  0.150908 &  0.216745 &  0.349859 &  0.157563 &  0.535667 &  0.221308 &  0.076762 &  0.199454 &  0.081964 &  0.364338 &  0.252603 &  - &  0.287454 &  0.508833 &  0.019770 &  0.002030 &  0.193610 &  0.545415 &  0.613478 &  0.367797 &  - \\
laser2 &  0.338900 &  - &  0.525555 &  0.585575 &  0.761541 &  0.567711 &  0.484499 &  0.258101 &  0.115246 &  0.223132 &  0.112247 &  0.345277 &  0.273463 &  - &  0.352930 &  0.559333 &  0.030970 &  0.007320 &  0.240160 &  0.649517 &  0.652654 &  0.698191 &  - \\
LaBSE &  0.385240 &  - &  0.604674 &  0.651042 &  0.841372 &  0.620106 &  0.547837 &  0.316038 &  0.206193 &  0.427871 &  0.282380 &  0.420933 &  0.348364 &  - &  0.495100 &  0.732833 &  0.197750 &  0.005750 &  0.500600 &  0.699400 &  0.779543 &  0.750975 &  - \\
all-MiniLM-L12-v2 &  0.275400 &  - &  0.448151 &  0.537626 &  0.755935 &  0.389383 &  0.460259 &  0.318294 &  0.195795 &  0.268374 &  0.207794 &  0.343522 &  0.292956 &  - &  0.457350 &  0.683333 &  0.331960 &  0.000760 &  0.581250 &  0.631624 &  0.695140 &  0.666773 &  - \\
all-MiniLM-L6-v2 &  0.268980 &  - &  0.426395 &  0.511567 &  0.750830 &  0.396524 &  0.518308 &  0.320659 &  0.188408 &  0.325805 &  0.217454 &  0.367358 &  0.281179 &  - &  0.316926 &  0.595667 &  0.284130 &  0.000000 &  0.573060 &  0.624823 &  0.770040 &  0.649303 &  - \\
distiluse-base-multilingual-cased-v2 &  0.357640 &  - &  0.598285 &  0.673874 &  0.849828 &  0.561071 &  0.559537 &  0.353854 &  0.182009 &  0.408716 &  0.245304 &  0.401705 &  0.346479 &  - &  0.517736 &  0.747833 &  0.269940 &  0.001710 &  0.620120 &  0.724944 &  0.764125 &  0.774883 &  - \\
multi-qa-MiniLM-L6-cos-v1 &  0.270460 &  - &  0.426429 &  0.499227 &  0.729690 &  0.371845 &  0.491319 &  0.261592 &  0.124914 &  0.352282 &  0.178171 &  0.351468 &  0.259531 &  - &  0.402797 &  0.650833 &  0.302290 &  0.000000 &  0.571530 &  0.621059 &  0.746188 &  0.638470 &  - \\
paraphrase-multilingual-MiniLM-L12-v2 &  0.367580 &  - &  0.575151 &  0.645192 &  0.776981 &  0.479361 &  0.560649 &  0.421582 &  0.232067 &  0.329181 &  0.274215 &  0.399715 &  0.365482 &  - &  0.490082 &  0.750333 &  0.266340 &  0.000690 &  0.629780 &  0.751024 &  0.705452 &  0.798982 &  - \\
sentence-t5-base &  0.373500 &  - &  0.511332 &  0.599193 &  0.750298 &  0.438459 &  0.584415 &  0.359335 &  0.177171 &  0.539211 &  0.283044 &  0.407692 &  0.300603 &  - &  0.501165 &  0.780500 &  0.275230 &  0.008180 &  0.630240 &  0.717363 &  0.776885 &  0.740406 &  - \\
sentence-t5-large &  0.414800 &  - &  0.570141 &  0.636012 &  0.795960 &  0.477294 &  0.618228 &  0.397757 &  0.187324 &  0.554836 &  0.263412 &  0.420726 &  0.318694 &  - &  0.579922 &  0.797667 &  0.345180 &  0.001770 &  0.700300 &  0.728274 &  0.750087 &  0.775924 &  - \\
sentence-t5-xl &  0.435160 &  - &  0.609852 &  0.664156 &  0.851425 &  0.543909 &  0.603725 &  0.407604 &  0.202789 &  0.536232 &  0.295641 &  0.416101 &  0.336037 &  - &  0.632994 &  0.830667 &  0.403750 &  0.009010 &  0.723410 &  0.750804 &  0.774935 &  0.794154 &  - \\
sentence-t5-xxl &  \textbf{0.460880} &  - &  \textbf{0.659079} &  0.685306 &  0.862011 &  0.583339 &  0.609771 &  0.435002 &  0.214049 &  0.530775 &  0.245417 &  0.422412 &  0.352475 &  - &  \textbf{0.683620} &  0.851500 &  0.457480 &  \textbf{0.055240} &  0.770850 &  0.770678 &  0.768024 &  0.812445 &  - \\
text2vec-base-multilingual &  0.342540 &  - &  0.519301 &  0.583087 &  0.718259 &  0.445349 &  0.491074 &  0.327224 &  0.161907 &  0.319305 &  0.193794 &  0.361904 &  0.303885 &  - &  0.514817 &  0.702833 &  0.188990 &  0.001970 &  0.463550 &  0.772481 &  0.740994 &  0.834760 &  - \\
text-embedding-ada-002 &  0.437640 &  - &  0.654203 &  0.711096 &  \textbf{0.893768} &  \textbf{0.644535} &  \textbf{0.648291} &  \textbf{0.535206} &  \textbf{0.261760} &  0.516655 &  \textbf{0.462086} &  0.445914 &  \textbf{0.416657} &  - &  - &  \textbf{0.898667} &  \textbf{0.516400} &  0.021510 &  \textbf{0.850370} &  0.762769 &  0.810931 &  0.775488 &  - \\
voyage-01 &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  0.472340 &  - &  0.795770 &  - &  - &  - &  - \\
voyage-02 &  0.357260 &  - &  0.539644 &  0.629691 &  0.802036 &  0.480770 &  - &  - &  - &  - &  - &  - &  - &  - &  0.573187 &  0.792167 &  0.379820 &  - &  0.676730 &  - &  - &  - &  - \\
voyage-lite-01 &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  0.485410 &  - &  0.688910 &  - &  - &  - &  - \\
MUSE-3 &  0.335140 &  - &  0.611903 &  0.702186 &  0.854964 &  0.539837 &  0.568992 &  0.378394 &  0.189473 &  0.508774 &  0.381532 &  0.438969 &  0.355014 &  - &  0.562253 &  0.738500 &  0.352670 &  0.000800 &  0.681510 &  0.713714 &  0.779122 &  0.754762 &  - \\
MUSE-large-3 &  0.350920 &  - &  0.658036 &  \textbf{0.734667} &  0.881867 &  0.636392 &  0.542089 &  0.379490 &  0.189434 &  0.417196 &  0.366391 &  0.410245 &  0.379674 &  - &  0.553932 &  0.771333 &  0.337810 &  0.000000 &  0.609910 &  0.743868 &  0.711062 &  0.781553 &  - \\
xlm-roberta-base &  0.267480 &  - &  0.135810 &  0.232145 &  0.438303 &  0.193768 &  0.522441 &  0.203748 &  0.086780 &  0.225000 &  0.070066 &  0.404430 &  0.241427 &  - &  0.255812 &  0.437500 &  0.001560 &  0.000000 &  0.004310 &  0.486154 &  0.567243 &  0.462263 &  - \\
xlm-roberta-large &  0.266160 &  - &  0.158204 &  0.239206 &  0.367711 &  0.153711 &  0.565361 &  0.211848 &  0.059433 &  0.269578 &  0.056710 &  0.426740 &  0.185013 &  - &  0.286153 &  0.494000 &  0.005170 &  0.000000 &  0.062660 &  0.500134 &  0.554916 &  0.423167 &  - \\
\end{tabular}
\end{table*}

